The composition rule for quantum systems is not the only possible one

Quantum theory provides a significant example of two intermingling hallmarks of science: the ability to consistently combine physical systems and study them compositely, and the power to extract predictions in the form of correlations. A striking consequence of this facet is the violation of Bell inequalities, which has been experimentally demonstrated via Bell tests. The prediction of this phenomenon originates as quantum systems are prescribed to combine according to the composition postulate, i.e. the tensor-product rule. This rule has also an operationally salient formulation given in terms of discriminability of composite states via local measurements. However, both the theoretical and the empirical status of such a postulate have been repeatedly challenged, questioning its independence from other physical principles -- most notably from quantum postulates pertaining solely to single systems. Is the composition postulate the only viable way to combine quantum systems into a consistent physical theory? Here, this long-standing problem is resolved by answering in the negative. This is achieved by adopting an operational approach to physical theories and exhibiting a family of theories that differ from standard quantum theory in their system-composition rule. These theories have the same predictions as standard quantum theory as far as Bell-like correlation scenarios are concerned. Quantum theory is thus established to embody genuinely more than quantum correlations. As a result, foundational programmes based on single-system principles only, or on mere Bell-like correlations, are operationally incomplete. On the experimental side, ascertaining the independence of postulates is a fundamental step to adjudicate between quantum theory and alternative physical theories: hence, the composition postulate calls for experimental scrutiny independently of the other features of quantum theory.

==> arxiv_lqt-v4/myqcircuit.tex <==
%    Q-circuit version 1.2
%    Copyright (C) 2004  Steve Flammia & Bryan Eastin, 4/23/06
%    This program is free software; you can redistribute it and/or modify
%    it under the terms of the GNU General Public License as published by
%    the Free Software Foundation; either version 2 of the License, or
%    (at your option) any later version.
%
%    This program is distributed in the hope that it will be useful,
%    but WITHOUT ANY WARRANTY; without even the implied warranty of
%    MERCHANTABILITY or FITNESS FOR A PARTICULAR PURPOSE.  See the
%    GNU General Public License for more details.
%
%    You should have received a copy of the GNU General Public License
%    along with this program; if not, write to the Free Software
%    Foundation, Inc., 59 Temple Place, Suite 330, Boston, MA  02111-1307  USA

\usepackage[matrix,frame,arrow]{xy}
\usepackage{amsmath}
\newcommand{\bra}[1]{\left\langle{#1}\right\vert}
\newcommand{\ket}[1]{\left\vert{#1}\right\rangle}
    % Defines Dirac notation.
\newcommand{\qw}[1][-1]{\ar @{-} [0,#1]}
    % Defines a wire that connects horizontally.  By default it connects to the object on the left of the current object.
    % WARNING: Wire commands must appear after the gate in any given entry.
\newcommand{\qwx}[1][-1]{\ar @{-} [#1,0]}
    % Defines a wire that connects vertically.  By default it connects to the object above the current object.
    % WARNING: Wire commands must appear after the gate in any given entry.
\newcommand{\cw}[1][-1]{\ar @{=} [0,#1]}
    % Defines a classical wire that connects horizontally.  By default it connects to the object on the left of the current object.
    % WARNING: Wire commands must appear after the gate in any given entry.
\newcommand{\cwx}[1][-1]{\ar @{=} [#1,0]}
    % Defines a classical wire that connects vertically.  By default it connects to the object above the current object.
    % WARNING: Wire commands must appear after the gate in any given entry.
\newcommand{\gate}[1]{*{\xy *+<.6em>{#1};p\save+LU;+RU **\dir{-}\restore\save+RU;+RD **\dir{-}\restore\save+RD;+LD **\dir{-}\restore\POS+LD;+LU **\dir{-}\endxy} \qw}
    % Boxes the argument, making a gate.
\newcommand{\meter}{\gate{\xy *!<0em,1.1em>h\cir<1.1em>{ur_dr},!U-<0em,.4em>;p+<.5em,.9em> **h\dir{-} \POS <-.6em,.4em> *{},<.6em,-.4em> *{} \endxy}}
    % Inserts a measurement meter.
\newcommand{\measure}[1]{*+[F-:<.9em>]{#1} \qw}
    % Inserts a measurement bubble with user defined text.
\newcommand{\measuretab}[1]{*{\xy *+<.6em>{#1};p\save+LU;+RU **\dir{-}\restore\save+RU;+RD **\dir{-}\restore\save+RD;+LD **\dir{-}\restore\save+LD;+LC-<.5em,0em> **\dir{-} \restore\POS+LU;+LC-<.5em,0em> **\dir{-} \endxy} \qw}
    % Inserts a measurement tab with user defined text.
\newcommand{\measureD}[1]{*{\xy*+=+<.5em>{\vphantom{\rule{0em}{.1em}#1}}*\cir{r_l};p\save*!R{#1} \restore\save+UC;+UC-<.5em,0em>*!R{\hphantom{#1}}+L **\dir{-} \restore\save+DC;+DC-<.5em,0em>*!R{\hphantom{#1}}+L **\dir{-} \restore\POS+UC-<.5em,0em>*!R{\hphantom{#1}}+L;+DC-<.5em,0em>*!R{\hphantom{#1}}+L **\dir{-} \endxy} \qw}
    % Inserts a D-shaped measurement gate with user defined text.
\newcommand{\multimeasure}[2]{*+<1em,.9em>{\hphantom{#2}} \qw \POS[0,0].[#1,0];p !C *{#2},p \drop\frm<.9em>{-}}
    % Draws a multiple qubit measurement bubble starting at the current position and spanning #1 additional gates below.
    % #2 gives the label for the gate.
    % You must use an argument of the same width as #2 in \ghost for the wires to connect properly on the lower lines.
\newcommand{\multimeasureD}[2]{*+<1em,.9em>{\hphantom{#2}}\save[0,0].[#1,0];p\save !C *{#2},p+LU+<0em,0em>;+RU+<-.8em,0em> **\dir{-}\restore\save +LD;+LU **\dir{-}\restore\save +LD;+RD-<.8em,0em> **\dir{-} \restore\save +RD+<0em,.8em>;+RU-<0em,.8em> **\dir{-} \restore \POS !UR*!UR{\cir<.9em>{r_d}};!DR*!DR{\cir<.9em>{d_l}}\restore \qw}
    % Draws a multiple qubit D-shaped measurement gate starting at the current position and spanning #1 additional gates below.
    % #2 gives the label for the gate.
    % You must use an argument of the same width as #2 in \ghost for the wires to connect properly on the lower lines.
\newcommand{\control}{*!<0em,.025em>-=-{\bullet}}
    % Inserts an unconnected control.
\newcommand{\controlo}{*-<.21em,.21em>{\xy *=<.59em>!<0em,-.02em>[o][F]{}\POS!C\endxy}}
    % Inserts a unconnected control-on-0.
\newcommand{\ctrl}[1]{\control \qwx[#1] \qw}
    % Inserts a control and connects it to the object #1 wires below.
\newcommand{\ctrlo}[1]{\controlo \qwx[#1] \qw}
    % Inserts a control-on-0 and connects it to the object #1 wires below.
\newcommand{\targ}{*!<0em,.019em>=<.79em,.68em>{\xy {<0em,0em>*{} \ar @{ - } +<.4em,0em> \ar @{ - } -<.4em,0em> \ar @{ - } +<0em,.36em> \ar @{ - } -<0em,.36em>},<0em,-.019em>*+<.8em>\frm{o}\endxy} \qw}
    % Inserts a CNOT target.
\newcommand{\qswap}{*=<0em>{\times} \qw}
    % Inserts half a swap gate. 
    % Must be connected to the other swap with \qwx.
\newcommand{\multigate}[2]{*+<1em,.9em>{\hphantom{#2}} \qw \POS[0,0].[#1,0];p !C *{#2},p \save+LU;+RU **\dir{-}\restore\save+RU;+RD **\dir{-}\restore\save+RD;+LD **\dir{-}\restore\save+LD;+LU **\dir{-}\restore}
    % Draws a multiple qubit gate starting at the current position and spanning #1 additional gates below.
    % #2 gives the label for the gate.
    % You must use an argument of the same width as #2 in \ghost for the wires to connect properly on the lower lines.
\newcommand{\ghost}[1]{*+<1em,.9em>{\hphantom{#1}} \qw}
    % Leaves space for \multigate on wires other than the one on which \multigate appears.  Without this command wires will cross your gate.
    % #1 should match the second argument in the corresponding \multigate. 
\newcommand{\push}[1]{*{#1}}
    % Inserts #1, overriding the default that causes entries to have zero size.  This command takes the place of a gate.
    % Like a gate, it must precede any wire commands.
    % \push is useful for forcing columns apart.
    % NOTE: It might be useful to know that a gate is about 1.3 times the height of its contents.  I.e. \gate{M} is 1.3em tall.
    % WARNING: \push must appear before any wire commands and may not appear in an entry with a gate or label.
\newcommand{\gategroup}[6]{\POS"#1,#2"."#3,#2"."#1,#4"."#3,#4"!C*+<#5>\frm{#6}}
    % Constructs a box or bracket enclosing the s % \begin{equation*}
%   \begin{aligned}
%     \Qcircuit @C=1em @R=.7em @! R {& \qw \poloFantasmaCn \sA & \multigate{1} 
% {\Transformation{A}_i \otimes \Transformation{B}_j} & \qw
%       \poloFantasmaCn \sB &\qw\\
%       & \qw \poloFantasmaCn \sC & \ghost {\Transformation{A}_i\otimes 
% \Transformation{B}_j} & \qw \poloFantasmaCn \sD &\qw}
%   \end{aligned}=
%   \begin{aligned}
%     \Qcircuit @C=1em @R=.7em @! R {& \qw \poloFantasmaCn \sA & \gate 
% {\Transformation{A}_i} & \qw \poloFantasmaCn \sB
%     &\qw\\ & \qw \poloFantasmaCn \sC & \gate{\Transformation{B}_j} & \qw 
% \poloFantasmaCn \sD &\qw}
%   \end{aligned}
% \end{equation*}quare block spanning rows #1-#3 and columns=#2-#4.
    % The block is given a margin #5/2, so #5 should be a valid length.
    % #6 can take the following arguments -- or . or _\} or ^\} or \{ or \} or _) or ^) or ( or ) where the first two options yield dashed and
    % dotted boxes respectively, and the last eight options yield bottom, top, left, and right braces of the curly or normal variety.
    % \gategroup can appear at the end of any gate entry, but it's good form to pick one of the corner gates.
    % BUG: \gategroup uses the four corner gates to determine the size of the bounding box.  Other gates may stick out of that box.  See \prop. 
\newcommand{\rstick}[1]{*!L!<-.5em,0em>=<0em>{#1}}
    % Centers the left side of #1 in the cell.  Intended for lining up wire labels.  Note that non-gates have default size zero.
\newcommand{\lstick}[1]{*!R!<.5em,0em>=<0em>{#1}}
    % Centers the right side of #1 in the cell.  Intended for lining up wire labels.  Note that non-gates have default size zero.
\newcommand{\ustick}[1]{*!D!<0em,-.5em>=<0em>{#1}}
    % Centers the bottom of #1 in the cell.  Intended for lining up wire labels.  Note that non-gates have default size zero.
\newcommand{\dstick}[1]{*!U!<0em,.5em>=<0em>{#1}}
    % Centers the top of #1 in the cell.  Intended for lining up wire labels.  Note that non-gates have default size zero.
\newcommand{\Qcircuit}[1][0em]{\xymatrix @*=<#1>}
    % Defines \Qcircuit as an \xymatrix with entries of default size 0em.  The optional argument, #1, is for use with clusters, and allows you
    % to fix the size of the nodes.  I would not advise using it with normal circuits.
\newcommand{\node}[2][]{{\begin{array}{c} \ _{#1}\  \\ {#2} \\ \ \end{array}}\drop\frm{o} }
    % When Qcircuit has been passed the optional argument for cluster states, this command produces a round node of the size specified in that
    % argument.  The optional argument #2 specifies the contents of a node, while optional argument #1 is a secondary label.  
\newcommand{\link}[2]{\ar @{-} [#1,#2]}
    % Draws a wire or connecting line to the element #1 rows down and #2 columns forward.
\newcommand{\pureghost}[1]{*+<1em,.9em>{\hphantom{#1}}}
    % Same as \ghost except it omits the wire leading to the left. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\multiprepareC}[2]{*+<1em,.9em>{\hphantom{#2}}\save[0,0].[#1,0];p\save !C
  *{#2},p+RU+<0em,0em>;+LU+<+.8em,0em> **\dir{-}\restore\save +RD;+RU **\dir{-}\restore\save
  +RD;+LD+<.8em,0em> **\dir{-} \restore\save +LD+<0em,.8em>;+LU-<0em,.8em> **\dir{-} \restore \POS
  !UL*!UL{\cir<.9em>{u_r}};!DL*!DL{\cir<.9em>{l_u}}\restore}
   % Draws a multiple qubit reverse-D-shaped preparation gate starting at the current position and spanning #1 additional gates below.
   % #2 gives the label for the gate.
   % You must use an argument of the same width as #2 in \pureghost for the wires to connect properly on
% the lower lines.
   % Inserts a reverse-D-shaped preparation gate with user defined text.
\newcommand{\prepareC}[1]{*{\xy*+=+<.5em>{\vphantom{#1\rule{0em}{.1em}}}*\cir{l^r};p\save*!L{#1} \restore\save+UC;+UC+<.5em,0em>*!L{\hphantom{#1}}+R **\dir{-} \restore\save+DC;+DC+<.5em,0em>*!L{\hphantom{#1}}+R **\dir{-} \restore\POS+UC+<.5em,0em>*!L{\hphantom{#1}}+R;+DC+<.5em,0em>*!L{\hphantom{#1}}+R **\dir{-} \endxy}}

\newcommand{\poloFantasmaCn}[1]{{{}^{#1}_{\phantom{#1}}}}


% Aggiunte di Franco


==> arxiv_lqt-v4/preamble.tex <==
\usepackage{url}
\def\UrlBreaks{\do\/\do-}
\usepackage{breakurl}
\usepackage{epsfig,amssymb,amsmath,mathrsfs,color}
\RequirePackage[colorlinks=true,linkcolor=blue,urlcolor=blue,citecolor=blue,linktocpage,breaklinks]{hyperref}
\usepackage{comment}
\usepackage{amsthm}
\def\bh{\mathbf{h}}
\def\<{\langle}\def\>{\rangle}
\def\rank{\operatorname{rank}}\def\Sym{\operatorname{Sym}}
\def\dist{\operatorname{dist}}\def\supp{\operatorname{Supp}}
\def\n#1{\|#1\|}
\def\sH{\mathcal{H}}
\def\Cmplx{\mathbb{C}}\def\Reals{\mathbb{R}}\def\N{\mathbb{N}}\def\Z{\mathbb{Z}}\def\M{\mathbb{M}}
\usepackage{hyperref}
\usepackage{enumerate}
\usepackage[shortlabels]{enumitem} %inline

\DeclareSymbolFont{sfletters}{OML}{cmbrm}{m}{it}
\DeclareMathSymbol{\srho}{\mathord}{sfletters}{"1A}
\DeclareMathSymbol{\svarrho}{\mathord}{sfletters}{"25}

\include{myqcircuit}

\newcommand{\ct}{\textsc{ct}}
\newcommand{\gpt}{\textsc{gpt}}
\newcommand{\gqt}{\textsc{gqt}}
\newcommand{\lqt}{\textsc{lqt}}
\newcommand{\bct}{\textsc{bct}}
\newcommand{\rqt}{\textsc{rqt}}
\newcommand{\fqt}{\textsc{fqt}}
\newcommand{\qt}{\textsc{qt}}
\newcommand{\nqt}{\textsc{nqt}}
\newcommand\bibit{bibit}
\newcommand{\rbra}[1]{({#1}\vert}
\newcommand{\rket}[1]{\vert{#1})}
\newcommand{\arbra}[1]{\left({#1}\right\vert}
\newcommand{\arket}[1]{\left\vert{#1}\right)}
\newcommand{\rbraket}[2]{( #1 \vphantom{#2} | #2 \vphantom{#1} )}
\newcommand{\arbraket}[2]{\left( #1 \vphantom{#2} \right|\left. #2 \vphantom{#1} \right)}

\theoremstyle{plain}
%\theoremstyle{remark}
\newtheorem*{definition*}{Definition}
\newtheorem{definition}{Definition}
\newtheorem{postulate}{Postulate}
\newtheorem{theorem}{Theorem}
\newtheorem*{theorem*}{Theorem}
\newtheorem{corollary}{Corollary}
\newtheorem*{corollary*}{Corollary}
\newtheorem*{proposition*}{Proposition}
\newtheorem{proposition}{Proposition}
\newtheorem{conjecture}{Conjecture}
\newtheorem*{conjecture*}{Conjecture}
\newtheorem*{question*}{Question}
\newtheorem{question}{Question}
\newtheorem*{problem*}{Problem}
\newtheorem{problem}{Problem}
\newtheorem*{lemma*}{Lemma}
\newtheorem{lemma}{Lemma}
\newtheorem*{example*}{Example}
\newtheorem{example}{Example}
\newtheorem{property}{Property}
\newtheorem*{property*}{Property}
\newtheorem*{remark*}{Remark}
\newtheorem{remark}{Remark}
\newtheorem*{proof*}{Proof}

\usepackage{graphicx}
\usepackage{epsfig}
\usepackage[color,matrix,frame,arrow]{xypic}
\vfuzz2pt
\usepackage{mathtools}
\usepackage{dsfont}
\usepackage{comment}
%\usepackage[font=small,labelfont=bf,
%   justification=justified,
%   format=plain]{caption}
%\usepackage[font=small,labelfont=bf,
%justification=justified,
%format=plain]{subcaption}
%\captionsetup[subfigure]{justification=justified,labelformat=simple}%,labelsep=colon}
%\renewcommand{\thesubfigure}{(\alph{subfigure})}

%\renewcommand{\v}[1]{\ensuremath{\mathbf{#1}}}
\newcommand{\gv}[1]{\ensuremath{\mbox{\boldmath$ #1 $}}} 
\newcommand{\braket}[2]{\left< #1 \vphantom{#2} | #2 \vphantom{#1} \right>}
%\newtheorem{lemma}{Lemma} \newtheorem{remark}{Remark} 
%\newtheorem{proposition}{Proposition}
%\newtheorem{example}{Example}
%\newtheorem*{example*}{Example}
%\newtheorem{corollary}{Corollary} \newtheorem{theorem}{Theorem}
 %\newtheorem{definition}{Definition}
\def\bvec#1{\mathbf{#1}}
\def\bk{\bvec k}
\def\bh{\bvec h}
\def\bik{{\bvec  k'}}
\def\bn{\bvec n} 
\def\bl{\bvec l} 
\def\bm{\bvec m}
\def\spc #1{{\mathsf #1}}
\def\Proof{\medskip\par\noindent{\bf Proof.  }}
\def\qed{$\,\blacksquare$\par} \def\>{\rangle} \def\<{\langle}
\def\kk{\>\! \>}\def\bb{\<\!\<} \def\map#1{\mathscr #1}
\def\lntrnsfrm#1{\mathrm #1} \def\sys#1{\mathrm{#1}} \def\rA{{\sys
    A}}\def\rB{{\sys B}}\def\rC{{\sys C}}\def\rD{{\sys D}}
\def\rE{{\sys E}} \def\rF{{\sys F}} \def\rG{{\sys G}} \def\rI{{\sys
    I}}\def\rc{{\sys c}} \def\rR{{\sys R}} \def\rS{{\sys
    S}}\def\rX{\sys X}\def\rY{\sys Y}\def\rZ{\sys Z}
\def\samp#1{\mathrm{#1}} \def\cX{{\samp X}} \def\cY{{\samp
    Y}}\def\cZ{{\samp Z}} \def\sH{{\spc H}} \def\sI{{\spc I}}
\def\tA{\map A}\def\tB{\map B}\def\tC{\map C}\def\tD{\map D}
\def\tS{\map S}\def\tG{\map G}\def\tL{\map L}\def\tK{\map K}
\def\tI{\map I}\def\tT{\map T}\def\tU{\map U} \def\tV{\map V}
\def\tW{\map W}\def\tM{\map M}\def\tX{\map X} \def\tY{\map
  Y}\def\tZ{\map Z}\def\tF{\map F}\def\tO{\map O}\def\tE{\map E}
\def\tJ{\map J}\def\tR{\map R}\def\tP{\map P }\def\tS{\map S}
\def\tT{\map T} \def\Cntset{\mathsf{Eff}} \def\grp#1{{\mathbf{#1}}}
\def\Span{\mathsf{Span}} \def\Stset{\mathsf{St}} \def\Trnset{{\mathsf
    T}} \def\K#1{\left|#1\right)\!}
\def\aff{\mathsf{Aff}}\def\con{\mathsf K}\def\det{\mathsf N}
\def\B#1{\left(#1\right|}
%  \def\SC#1#2{\left({#1}\right|\left.\!{#2}\right)\!}  
\def\Tr{{\rm Tr}} \def\Eta{\rm{H}} \def\Reals{{\mathbb R}}
\def\ch{\ensuremath{\mathfrak{C}}} \def\cu{\ensuremath{\mathsf C}}
\newcommand\remind[1]{\marginpar{\baselineskip=6pt$\blacktriangleright$
    \raggedright{\tiny #1 }}}
\newcommand\marginlabel[1]{\marginpar{#1}}

\usepackage[usenames,dvipsnames]{xcolor}
\def\nota#1{\textcolor{BurntOrange}{\textbf{#1}}}
\usepackage{soul}

\newcommand{\ExtSt}[1]{\ensuremath{\mathsf{ExtSt}(\mathrm{#1})}}
\newcommand{\ExtStZ}[1]{\ensuremath{\mathsf{ExtSt}_0(\mathrm{#1})}}
\newcommand{\s}[1]{\ustick{\scriptstyle{\sys{#1}}}}
\newcommand{\Sys}[1]{\ensuremath{\mathsf{Sys(\mathrm{#1})}}}
\newcommand{\Ob}[1]{\ensuremath{\mathsf{Ob(\mathrm{#1})}}}
\newcommand{\syst}[1]{\ensuremath{\mathrm{#1}}}
\newcommand{\D}[1]{\ensuremath{D_\syst{#1}}}
\newcommand{\St}[1]{\ensuremath{\mathsf{St(\mathrm{#1})}}}
\newcommand{\StC}[1]{\ensuremath{\mathsf{St_+(\mathrm{#1})}}}
\newcommand{\StN}[1]{\ensuremath{\mathsf{St_1(\mathrm{#1})}}}
\newcommand{\StR}[1]{\ensuremath{\mathsf{St}_{\mathbb{R}}(\mathrm{#1})}}
\newcommand{\C}[1]{\ensuremath{\mathsf{S(\mathrm{#1})}}}
\newcommand{\PurSt}[1]{\ensuremath{\mathsf{PurSt(\mathrm{#1})}}}
\newcommand{\PurRef}[2]{\ensuremath{\mathsf{PurRef}_{#1}(\mathrm{#2})}}
\newcommand{\PurRefA}[1]{\ensuremath{\mathsf{PurRef}(\mathrm{#1})}}
\newcommand{\PurRefbar}[1]{\ensuremath{\overline{\mathsf{PurRef}}(\mathrm{#1})}}
\newcommand{\PS}[1]{\ensuremath{\mathsf{PrSt(\mathrm{#1})}}}
\newcommand{\ConvH}[1]{\ensuremath{\mathsf{ConvH(#1)}}}
\newcommand{\Eff}[1]{\ensuremath{\mathsf{Eff(\mathrm{#1})}}}
\newcommand{\EffR}[1]{\ensuremath{\mathsf{Eff}_{\mathbb{R}}(\mathrm{#1})}}
\newcommand{\EffC}[1]{\ensuremath{\mathsf{Eff_+(\mathrm{#1})}}}
\newcommand{\EffN}[1]{\ensuremath{\mathsf{Eff_1(\mathrm{#1})}}}
\newcommand{\E}[1]{\ensuremath{\mathsf{E(\mathrm{#1})}}}
\newcommand{\T}[1]{\ensuremath{\mathcal{#1}}}
\newcommand{\Transf}[2]{\ensuremath{\mathsf{Transf(\mathrm{#1}\!\to\!\mathrm{#2})}}}
\newcommand{\TransfR}[2]{\ensuremath{\mathsf{Transf_{\mathbb{R}}(\mathrm{#1}\!\to\!\mathrm{#2})}}}
\newcommand{\TransfN}[2]{\ensuremath{\mathsf{Transf_{1}(\mathrm{#1}\!\to\!\mathrm{#2})}}}
\newcommand{\TransfC}[2]{\ensuremath{\mathsf{Transf_{+}(\mathrm{#1}\!\to\!\mathrm{#2})}}}
\newcommand{\transf}[1]{\ensuremath{\mathsf{Transf(\mathrm{#1})}}}
\newcommand{\Mor}[2]{\ensuremath{\mathsf{Mor(\mathrm{#1}\!\to\!\mathrm{#2})}}}
\newcommand{\mor}[1]{\ensuremath{\mathsf{Mor(\mathrm{#1})}}}
\newcommand{\TransfA}[1]{\ensuremath{\mathsf{Transf(\mathrm{#1})}}}
\newcommand{\RevTransfA}[1]{\ensuremath{\mathsf{RevTransf(\mathrm{#1})}}}
\newcommand{\RevTransf}[2]{\ensuremath{\mathsf{RevTransf(\mathrm{#1}\!\to\!\mathrm{#2})}}}
\newcommand{\LocTransf}[2]{\ensuremath{\mathsf{LocTransf(\mathrm{#1}\!\to\!\mathrm{#2})}}}
\newcommand{\LocTransfA}[1]{\ensuremath{\mathsf{LocTransf(\mathrm{#1})}}}
\newcommand{\TestC}[4]{\ensuremath{\mathsf{#1}_{\mathsf{#2}}^{\mathrm{#3}\!\to\!\mathrm{#4}}}}
\newcommand{\TestAB}[2]{\ensuremath{\mathsf{Test(\mathrm{#1}\!\to\!\mathrm{#2})}}}
\newcommand{\Test}[2]{\ensuremath{\mathsf{#1_{\mathsf{#2}}}}}
\newcommand{\TestA}[1]{\ensuremath{\mathsf{Test(\mathrm{#1})}}}
\newcommand{\InstrC}[4]{\ensuremath{\mathsf{#1}_{\mathsf{#2}}^{\mathrm{#3}\!\to\!\mathrm{#4}}}}
\newcommand{\InstrAB}[2]{\ensuremath{\mathsf{Instr(\mathrm{#1}\!\to\!\mathrm{#2})}}}
\newcommand{\InstrABR}[2]{\ensuremath{\mathsf{Instr_{\mathbb{R}}(\mathrm{#1}\!\to\!\mathrm{#2})}}}
\newcommand{\Instr}[2]{\ensuremath{\mathsf{#1_{\mathsf{#2}}}}}
\newcommand{\InstrA}[1]{\ensuremath{\mathsf{Instr(\mathrm{#1})}}}
\newcommand{\Event}[2]{\ensuremath{\mathsf{Event(\mathrm{#1}\!\to\!\mathrm{#2})}}}
\newcommand{\EventA}[1]{\ensuremath{\mathsf{Event(\mathrm{#1})}}}
\newcommand{\Out}[1]{\ensuremath{\mathsf{#1}}}
\newcommand{\Refi}[1]{\ensuremath{\mathsf{Ref}(\mathscr{#1})}}
\newcommand{\ConvRef}[1]{\ensuremath{\mathsf{ConvRef(\mathscr{#1})}}}

\usepackage{tikz}
\input{tikzit.sty}
\input{style.tikzstyles}

\usepackage{stmaryrd}
\usepackage{xpatch}

\makeatletter
\patchcmd{\@ssect@ltx}
{\addcontentsline{toc}{#1}{\protect\numberline{}#8}}
{}
{}
{}
\makeatother

\makeatletter
\def\@bibdataout@aps{%
	\immediate\write\@bibdataout{%
		@CONTROL{%
			apsrev41Control%
			\longbibliography@sw{%
				,author="08",editor="1",pages="1",title="0",year="1"%
			}{%
				,author="08",editor="1",pages="1",title="",year="1"%
			}%
		}%
	}%
	\if@filesw \immediate \write \@auxout {\string \citation {apsrev41Control}}\fi 
}
\makeatother

==> myqcircuit.tex <==
%    Q-circuit version 1.2
%    Copyright (C) 2004  Steve Flammia & Bryan Eastin, 4/23/06
%    This program is free software; you can redistribute it and/or modify
%    it under the terms of the GNU General Public License as published by
%    the Free Software Foundation; either version 2 of the License, or
%    (at your option) any later version.
%
%    This program is distributed in the hope that it will be useful,
%    but WITHOUT ANY WARRANTY; without even the implied warranty of
%    MERCHANTABILITY or FITNESS FOR A PARTICULAR PURPOSE.  See the
%    GNU General Public License for more details.
%
%    You should have received a copy of the GNU General Public License
%    along with this program; if not, write to the Free Software
%    Foundation, Inc., 59 Temple Place, Suite 330, Boston, MA  02111-1307  USA

\usepackage[matrix,frame,arrow]{xy}
\usepackage{amsmath}
\newcommand{\bra}[1]{\left\langle{#1}\right\vert}
\newcommand{\ket}[1]{\left\vert{#1}\right\rangle}
    % Defines Dirac notation.
\newcommand{\qw}[1][-1]{\ar @{-} [0,#1]}
    % Defines a wire that connects horizontally.  By default it connects to the object on the left of the current object.
    % WARNING: Wire commands must appear after the gate in any given entry.
\newcommand{\qwx}[1][-1]{\ar @{-} [#1,0]}
    % Defines a wire that connects vertically.  By default it connects to the object above the current object.
    % WARNING: Wire commands must appear after the gate in any given entry.
\newcommand{\cw}[1][-1]{\ar @{=} [0,#1]}
    % Defines a classical wire that connects horizontally.  By default it connects to the object on the left of the current object.
    % WARNING: Wire commands must appear after the gate in any given entry.
\newcommand{\cwx}[1][-1]{\ar @{=} [#1,0]}
    % Defines a classical wire that connects vertically.  By default it connects to the object above the current object.
    % WARNING: Wire commands must appear after the gate in any given entry.
\newcommand{\gate}[1]{*{\xy *+<.6em>{#1};p\save+LU;+RU **\dir{-}\restore\save+RU;+RD **\dir{-}\restore\save+RD;+LD **\dir{-}\restore\POS+LD;+LU **\dir{-}\endxy} \qw}
    % Boxes the argument, making a gate.
\newcommand{\meter}{\gate{\xy *!<0em,1.1em>h\cir<1.1em>{ur_dr},!U-<0em,.4em>;p+<.5em,.9em> **h\dir{-} \POS <-.6em,.4em> *{},<.6em,-.4em> *{} \endxy}}
    % Inserts a measurement meter.
\newcommand{\measure}[1]{*+[F-:<.9em>]{#1} \qw}
    % Inserts a measurement bubble with user defined text.
\newcommand{\measuretab}[1]{*{\xy *+<.6em>{#1};p\save+LU;+RU **\dir{-}\restore\save+RU;+RD **\dir{-}\restore\save+RD;+LD **\dir{-}\restore\save+LD;+LC-<.5em,0em> **\dir{-} \restore\POS+LU;+LC-<.5em,0em> **\dir{-} \endxy} \qw}
    % Inserts a measurement tab with user defined text.
\newcommand{\measureD}[1]{*{\xy*+=+<.5em>{\vphantom{\rule{0em}{.1em}#1}}*\cir{r_l};p\save*!R{#1} \restore\save+UC;+UC-<.5em,0em>*!R{\hphantom{#1}}+L **\dir{-} \restore\save+DC;+DC-<.5em,0em>*!R{\hphantom{#1}}+L **\dir{-} \restore\POS+UC-<.5em,0em>*!R{\hphantom{#1}}+L;+DC-<.5em,0em>*!R{\hphantom{#1}}+L **\dir{-} \endxy} \qw}
    % Inserts a D-shaped measurement gate with user defined text.
\newcommand{\multimeasure}[2]{*+<1em,.9em>{\hphantom{#2}} \qw \POS[0,0].[#1,0];p !C *{#2},p \drop\frm<.9em>{-}}
    % Draws a multiple qubit measurement bubble starting at the current position and spanning #1 additional gates below.
    % #2 gives the label for the gate.
    % You must use an argument of the same width as #2 in \ghost for the wires to connect properly on the lower lines.
\newcommand{\multimeasureD}[2]{*+<1em,.9em>{\hphantom{#2}}\save[0,0].[#1,0];p\save !C *{#2},p+LU+<0em,0em>;+RU+<-.8em,0em> **\dir{-}\restore\save +LD;+LU **\dir{-}\restore\save +LD;+RD-<.8em,0em> **\dir{-} \restore\save +RD+<0em,.8em>;+RU-<0em,.8em> **\dir{-} \restore \POS !UR*!UR{\cir<.9em>{r_d}};!DR*!DR{\cir<.9em>{d_l}}\restore \qw}
    % Draws a multiple qubit D-shaped measurement gate starting at the current position and spanning #1 additional gates below.
    % #2 gives the label for the gate.
    % You must use an argument of the same width as #2 in \ghost for the wires to connect properly on the lower lines.
\newcommand{\control}{*!<0em,.025em>-=-{\bullet}}
    % Inserts an unconnected control.
\newcommand{\controlo}{*-<.21em,.21em>{\xy *=<.59em>!<0em,-.02em>[o][F]{}\POS!C\endxy}}
    % Inserts a unconnected control-on-0.
\newcommand{\ctrl}[1]{\control \qwx[#1] \qw}
    % Inserts a control and connects it to the object #1 wires below.
\newcommand{\ctrlo}[1]{\controlo \qwx[#1] \qw}
    % Inserts a control-on-0 and connects it to the object #1 wires below.
\newcommand{\targ}{*!<0em,.019em>=<.79em,.68em>{\xy {<0em,0em>*{} \ar @{ - } +<.4em,0em> \ar @{ - } -<.4em,0em> \ar @{ - } +<0em,.36em> \ar @{ - } -<0em,.36em>},<0em,-.019em>*+<.8em>\frm{o}\endxy} \qw}
    % Inserts a CNOT target.
\newcommand{\qswap}{*=<0em>{\times} \qw}
    % Inserts half a swap gate. 
    % Must be connected to the other swap with \qwx.
\newcommand{\multigate}[2]{*+<1em,.9em>{\hphantom{#2}} \qw \POS[0,0].[#1,0];p !C *{#2},p \save+LU;+RU **\dir{-}\restore\save+RU;+RD **\dir{-}\restore\save+RD;+LD **\dir{-}\restore\save+LD;+LU **\dir{-}\restore}
    % Draws a multiple qubit gate starting at the current position and spanning #1 additional gates below.
    % #2 gives the label for the gate.
    % You must use an argument of the same width as #2 in \ghost for the wires to connect properly on the lower lines.
\newcommand{\ghost}[1]{*+<1em,.9em>{\hphantom{#1}} \qw}
    % Leaves space for \multigate on wires other than the one on which \multigate appears.  Without this command wires will cross your gate.
    % #1 should match the second argument in the corresponding \multigate. 
\newcommand{\push}[1]{*{#1}}
    % Inserts #1, overriding the default that causes entries to have zero size.  This command takes the place of a gate.
    % Like a gate, it must precede any wire commands.
    % \push is useful for forcing columns apart.
    % NOTE: It might be useful to know that a gate is about 1.3 times the height of its contents.  I.e. \gate{M} is 1.3em tall.
    % WARNING: \push must appear before any wire commands and may not appear in an entry with a gate or label.
\newcommand{\gategroup}[6]{\POS"#1,#2"."#3,#2"."#1,#4"."#3,#4"!C*+<#5>\frm{#6}}
    % Constructs a box or bracket enclosing the s % \begin{equation*}
%   \begin{aligned}
%     \Qcircuit @C=1em @R=.7em @! R {& \qw \poloFantasmaCn \sA & \multigate{1} 
% {\Transformation{A}_i \otimes \Transformation{B}_j} & \qw
%       \poloFantasmaCn \sB &\qw\\
%       & \qw \poloFantasmaCn \sC & \ghost {\Transformation{A}_i\otimes 
% \Transformation{B}_j} & \qw \poloFantasmaCn \sD &\qw}
%   \end{aligned}=
%   \begin{aligned}
%     \Qcircuit @C=1em @R=.7em @! R {& \qw \poloFantasmaCn \sA & \gate 
% {\Transformation{A}_i} & \qw \poloFantasmaCn \sB
%     &\qw\\ & \qw \poloFantasmaCn \sC & \gate{\Transformation{B}_j} & \qw 
% \poloFantasmaCn \sD &\qw}
%   \end{aligned}
% \end{equation*}quare block spanning rows #1-#3 and columns=#2-#4.
    % The block is given a margin #5/2, so #5 should be a valid length.
    % #6 can take the following arguments -- or . or _\} or ^\} or \{ or \} or _) or ^) or ( or ) where the first two options yield dashed and
    % dotted boxes respectively, and the last eight options yield bottom, top, left, and right braces of the curly or normal variety.
    % \gategroup can appear at the end of any gate entry, but it's good form to pick one of the corner gates.
    % BUG: \gategroup uses the four corner gates to determine the size of the bounding box.  Other gates may stick out of that box.  See \prop. 
\newcommand{\rstick}[1]{*!L!<-.5em,0em>=<0em>{#1}}
    % Centers the left side of #1 in the cell.  Intended for lining up wire labels.  Note that non-gates have default size zero.
\newcommand{\lstick}[1]{*!R!<.5em,0em>=<0em>{#1}}
    % Centers the right side of #1 in the cell.  Intended for lining up wire labels.  Note that non-gates have default size zero.
\newcommand{\ustick}[1]{*!D!<0em,-.5em>=<0em>{#1}}
    % Centers the bottom of #1 in the cell.  Intended for lining up wire labels.  Note that non-gates have default size zero.
\newcommand{\dstick}[1]{*!U!<0em,.5em>=<0em>{#1}}
    % Centers the top of #1 in the cell.  Intended for lining up wire labels.  Note that non-gates have default size zero.
\newcommand{\Qcircuit}[1][0em]{\xymatrix @*=<#1>}
    % Defines \Qcircuit as an \xymatrix with entries of default size 0em.  The optional argument, #1, is for use with clusters, and allows you
    % to fix the size of the nodes.  I would not advise using it with normal circuits.
\newcommand{\node}[2][]{{\begin{array}{c} \ _{#1}\  \\ {#2} \\ \ \end{array}}\drop\frm{o} }
    % When Qcircuit has been passed the optional argument for cluster states, this command produces a round node of the size specified in that
    % argument.  The optional argument #2 specifies the contents of a node, while optional argument #1 is a secondary label.  
\newcommand{\link}[2]{\ar @{-} [#1,#2]}
    % Draws a wire or connecting line to the element #1 rows down and #2 columns forward.
\newcommand{\pureghost}[1]{*+<1em,.9em>{\hphantom{#1}}}
    % Same as \ghost except it omits the wire leading to the left. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\multiprepareC}[2]{*+<1em,.9em>{\hphantom{#2}}\save[0,0].[#1,0];p\save !C
  *{#2},p+RU+<0em,0em>;+LU+<+.8em,0em> **\dir{-}\restore\save +RD;+RU **\dir{-}\restore\save
  +RD;+LD+<.8em,0em> **\dir{-} \restore\save +LD+<0em,.8em>;+LU-<0em,.8em> **\dir{-} \restore \POS
  !UL*!UL{\cir<.9em>{u_r}};!DL*!DL{\cir<.9em>{l_u}}\restore}
   % Draws a multiple qubit reverse-D-shaped preparation gate starting at the current position and spanning #1 additional gates below.
   % #2 gives the label for the gate.
   % You must use an argument of the same width as #2 in \pureghost for the wires to connect properly on
% the lower lines.
   % Inserts a reverse-D-shaped preparation gate with user defined text.
\newcommand{\prepareC}[1]{*{\xy*+=+<.5em>{\vphantom{#1\rule{0em}{.1em}}}*\cir{l^r};p\save*!L{#1} \restore\save+UC;+UC+<.5em,0em>*!L{\hphantom{#1}}+R **\dir{-} \restore\save+DC;+DC+<.5em,0em>*!L{\hphantom{#1}}+R **\dir{-} \restore\POS+UC+<.5em,0em>*!L{\hphantom{#1}}+R;+DC+<.5em,0em>*!L{\hphantom{#1}}+R **\dir{-} \endxy}}

\newcommand{\poloFantasmaCn}[1]{{{}^{#1}_{\phantom{#1}}}}


% Aggiunte di Franco


==> preamble.tex <==
\usepackage{url}
\def\UrlBreaks{\do\/\do-}
\usepackage{breakurl}
\usepackage{epsfig,amssymb,amsmath,mathrsfs,color}
\RequirePackage[colorlinks=true,linkcolor=blue,urlcolor=blue,citecolor=blue,linktocpage,breaklinks]{hyperref}
\usepackage{comment}
\usepackage{amsthm}
\def\bh{\mathbf{h}}
\def\<{\langle}\def\>{\rangle}
\def\rank{\operatorname{rank}}\def\Sym{\operatorname{Sym}}
\def\dist{\operatorname{dist}}\def\supp{\operatorname{Supp}}
\def\n#1{\|#1\|}
\def\sH{\mathcal{H}}
\def\Cmplx{\mathbb{C}}\def\Reals{\mathbb{R}}\def\N{\mathbb{N}}\def\Z{\mathbb{Z}}\def\M{\mathbb{M}}
\usepackage{hyperref}
\usepackage{enumerate}
\usepackage[shortlabels]{enumitem} %inline

\DeclareSymbolFont{sfletters}{OML}{cmbrm}{m}{it}
\DeclareMathSymbol{\srho}{\mathord}{sfletters}{"1A}
\DeclareMathSymbol{\svarrho}{\mathord}{sfletters}{"25}

\include{myqcircuit}

\newcommand{\ct}{\textsc{ct}}
\newcommand{\gpt}{\textsc{gpt}}
\newcommand{\gqt}{\textsc{gqt}}
\newcommand{\lqt}{\textsc{lqt}}
\newcommand{\bct}{\textsc{bct}}
\newcommand{\rqt}{\textsc{rqt}}
\newcommand{\fqt}{\textsc{fqt}}
\newcommand{\qt}{\textsc{qt}}
\newcommand{\nqt}{\textsc{nqt}}
\newcommand\bibit{bibit}
\newcommand{\rbra}[1]{({#1}\vert}
\newcommand{\rket}[1]{\vert{#1})}
\newcommand{\arbra}[1]{\left({#1}\right\vert}
\newcommand{\arket}[1]{\left\vert{#1}\right)}
\newcommand{\rbraket}[2]{( #1 \vphantom{#2} | #2 \vphantom{#1} )}
\newcommand{\arbraket}[2]{\left( #1 \vphantom{#2} \right|\left. #2 \vphantom{#1} \right)}

\theoremstyle{plain}
%\theoremstyle{remark}
\newtheorem*{definition*}{Definition}
\newtheorem{definition}{Definition}
\newtheorem{postulate}{Postulate}
\newtheorem{theorem}{Theorem}
\newtheorem*{theorem*}{Theorem}
\newtheorem{corollary}{Corollary}
\newtheorem*{corollary*}{Corollary}
\newtheorem*{proposition*}{Proposition}
\newtheorem{proposition}{Proposition}
\newtheorem{conjecture}{Conjecture}
\newtheorem*{conjecture*}{Conjecture}
\newtheorem*{question*}{Question}
\newtheorem{question}{Question}
\newtheorem*{problem*}{Problem}
\newtheorem{problem}{Problem}
\newtheorem*{lemma*}{Lemma}
\newtheorem{lemma}{Lemma}
\newtheorem*{example*}{Example}
\newtheorem{example}{Example}
\newtheorem{property}{Property}
\newtheorem*{property*}{Property}
\newtheorem*{remark*}{Remark}
\newtheorem{remark}{Remark}
\newtheorem*{proof*}{Proof}

\usepackage{graphicx}
\usepackage{epsfig}
\usepackage[color,matrix,frame,arrow]{xypic}
\vfuzz2pt
\usepackage{mathtools}
\usepackage{dsfont}
\usepackage{comment}
%\usepackage[font=small,labelfont=bf,
%   justification=justified,
%   format=plain]{caption}
%\usepackage[font=small,labelfont=bf,
%justification=justified,
%format=plain]{subcaption}
%\captionsetup[subfigure]{justification=justified,labelformat=simple}%,labelsep=colon}
%\renewcommand{\thesubfigure}{(\alph{subfigure})}

%\renewcommand{\v}[1]{\ensuremath{\mathbf{#1}}}
\newcommand{\gv}[1]{\ensuremath{\mbox{\boldmath$ #1 $}}} 
\newcommand{\braket}[2]{\left< #1 \vphantom{#2} | #2 \vphantom{#1} \right>}
%\newtheorem{lemma}{Lemma} \newtheorem{remark}{Remark} 
%\newtheorem{proposition}{Proposition}
%\newtheorem{example}{Example}
%\newtheorem*{example*}{Example}
%\newtheorem{corollary}{Corollary} \newtheorem{theorem}{Theorem}
 %\newtheorem{definition}{Definition}
\def\bvec#1{\mathbf{#1}}
\def\bk{\bvec k}
\def\bh{\bvec h}
\def\bik{{\bvec  k'}}
\def\bn{\bvec n} 
\def\bl{\bvec l} 
\def\bm{\bvec m}
\def\spc #1{{\mathsf #1}}
\def\Proof{\medskip\par\noindent{\bf Proof.  }}
\def\qed{$\,\blacksquare$\par} \def\>{\rangle} \def\<{\langle}
\def\kk{\>\! \>}\def\bb{\<\!\<} \def\map#1{\mathscr #1}
\def\lntrnsfrm#1{\mathrm #1} \def\sys#1{\mathrm{#1}} \def\rA{{\sys
    A}}\def\rB{{\sys B}}\def\rC{{\sys C}}\def\rD{{\sys D}}
\def\rE{{\sys E}} \def\rF{{\sys F}} \def\rG{{\sys G}} \def\rI{{\sys
    I}}\def\rc{{\sys c}} \def\rR{{\sys R}} \def\rS{{\sys
    S}}\def\rX{\sys X}\def\rY{\sys Y}\def\rZ{\sys Z}
\def\samp#1{\mathrm{#1}} \def\cX{{\samp X}} \def\cY{{\samp
    Y}}\def\cZ{{\samp Z}} \def\sH{{\spc H}} \def\sI{{\spc I}}
\def\tA{\map A}\def\tB{\map B}\def\tC{\map C}\def\tD{\map D}
\def\tS{\map S}\def\tG{\map G}\def\tL{\map L}\def\tK{\map K}
\def\tI{\map I}\def\tT{\map T}\def\tU{\map U} \def\tV{\map V}
\def\tW{\map W}\def\tM{\map M}\def\tX{\map X} \def\tY{\map
  Y}\def\tZ{\map Z}\def\tF{\map F}\def\tO{\map O}\def\tE{\map E}
\def\tJ{\map J}\def\tR{\map R}\def\tP{\map P }\def\tS{\map S}
\def\tT{\map T} \def\Cntset{\mathsf{Eff}} \def\grp#1{{\mathbf{#1}}}
\def\Span{\mathsf{Span}} \def\Stset{\mathsf{St}} \def\Trnset{{\mathsf
    T}} \def\K#1{\left|#1\right)\!}
\def\aff{\mathsf{Aff}}\def\con{\mathsf K}\def\det{\mathsf N}
\def\B#1{\left(#1\right|}
%  \def\SC#1#2{\left({#1}\right|\left.\!{#2}\right)\!}  
\def\Tr{{\rm Tr}} \def\Eta{\rm{H}} \def\Reals{{\mathbb R}}
\def\ch{\ensuremath{\mathfrak{C}}} \def\cu{\ensuremath{\mathsf C}}
\newcommand\remind[1]{\marginpar{\baselineskip=6pt$\blacktriangleright$
    \raggedright{\tiny #1 }}}
\newcommand\marginlabel[1]{\marginpar{#1}}

\usepackage[usenames,dvipsnames]{xcolor}
\def\nota#1{\textcolor{BurntOrange}{\textbf{#1}}}
\usepackage{soul}

\newcommand{\ExtSt}[1]{\ensuremath{\mathsf{ExtSt}(\mathrm{#1})}}
\newcommand{\ExtStZ}[1]{\ensuremath{\mathsf{ExtSt}_0(\mathrm{#1})}}
\newcommand{\s}[1]{\ustick{\scriptstyle{\sys{#1}}}}
\newcommand{\Sys}[1]{\ensuremath{\mathsf{Sys(\mathrm{#1})}}}
\newcommand{\Ob}[1]{\ensuremath{\mathsf{Ob(\mathrm{#1})}}}
\newcommand{\syst}[1]{\ensuremath{\mathrm{#1}}}
\newcommand{\D}[1]{\ensuremath{D_\syst{#1}}}
\newcommand{\St}[1]{\ensuremath{\mathsf{St(\mathrm{#1})}}}
\newcommand{\StC}[1]{\ensuremath{\mathsf{St_+(\mathrm{#1})}}}
\newcommand{\StN}[1]{\ensuremath{\mathsf{St_1(\mathrm{#1})}}}
\newcommand{\StR}[1]{\ensuremath{\mathsf{St}_{\mathbb{R}}(\mathrm{#1})}}
\newcommand{\C}[1]{\ensuremath{\mathsf{S(\mathrm{#1})}}}
\newcommand{\PurSt}[1]{\ensuremath{\mathsf{PurSt(\mathrm{#1})}}}
\newcommand{\PurRef}[2]{\ensuremath{\mathsf{PurRef}_{#1}(\mathrm{#2})}}
\newcommand{\PurRefA}[1]{\ensuremath{\mathsf{PurRef}(\mathrm{#1})}}
\newcommand{\PurRefbar}[1]{\ensuremath{\overline{\mathsf{PurRef}}(\mathrm{#1})}}
\newcommand{\PS}[1]{\ensuremath{\mathsf{PrSt(\mathrm{#1})}}}
\newcommand{\ConvH}[1]{\ensuremath{\mathsf{ConvH(#1)}}}
\newcommand{\Eff}[1]{\ensuremath{\mathsf{Eff(\mathrm{#1})}}}
\newcommand{\EffR}[1]{\ensuremath{\mathsf{Eff}_{\mathbb{R}}(\mathrm{#1})}}
\newcommand{\EffC}[1]{\ensuremath{\mathsf{Eff_+(\mathrm{#1})}}}
\newcommand{\EffN}[1]{\ensuremath{\mathsf{Eff_1(\mathrm{#1})}}}
\newcommand{\E}[1]{\ensuremath{\mathsf{E(\mathrm{#1})}}}
\newcommand{\T}[1]{\ensuremath{\mathcal{#1}}}
\newcommand{\Transf}[2]{\ensuremath{\mathsf{Transf(\mathrm{#1}\!\to\!\mathrm{#2})}}}
\newcommand{\TransfR}[2]{\ensuremath{\mathsf{Transf_{\mathbb{R}}(\mathrm{#1}\!\to\!\mathrm{#2})}}}
\newcommand{\TransfN}[2]{\ensuremath{\mathsf{Transf_{1}(\mathrm{#1}\!\to\!\mathrm{#2})}}}
\newcommand{\TransfC}[2]{\ensuremath{\mathsf{Transf_{+}(\mathrm{#1}\!\to\!\mathrm{#2})}}}
\newcommand{\transf}[1]{\ensuremath{\mathsf{Transf(\mathrm{#1})}}}
\newcommand{\Mor}[2]{\ensuremath{\mathsf{Mor(\mathrm{#1}\!\to\!\mathrm{#2})}}}
\newcommand{\mor}[1]{\ensuremath{\mathsf{Mor(\mathrm{#1})}}}
\newcommand{\TransfA}[1]{\ensuremath{\mathsf{Transf(\mathrm{#1})}}}
\newcommand{\RevTransfA}[1]{\ensuremath{\mathsf{RevTransf(\mathrm{#1})}}}
\newcommand{\RevTransf}[2]{\ensuremath{\mathsf{RevTransf(\mathrm{#1}\!\to\!\mathrm{#2})}}}
\newcommand{\LocTransf}[2]{\ensuremath{\mathsf{LocTransf(\mathrm{#1}\!\to\!\mathrm{#2})}}}
\newcommand{\LocTransfA}[1]{\ensuremath{\mathsf{LocTransf(\mathrm{#1})}}}
\newcommand{\TestC}[4]{\ensuremath{\mathsf{#1}_{\mathsf{#2}}^{\mathrm{#3}\!\to\!\mathrm{#4}}}}
\newcommand{\TestAB}[2]{\ensuremath{\mathsf{Test(\mathrm{#1}\!\to\!\mathrm{#2})}}}
\newcommand{\Test}[2]{\ensuremath{\mathsf{#1_{\mathsf{#2}}}}}
\newcommand{\TestA}[1]{\ensuremath{\mathsf{Test(\mathrm{#1})}}}
\newcommand{\InstrC}[4]{\ensuremath{\mathsf{#1}_{\mathsf{#2}}^{\mathrm{#3}\!\to\!\mathrm{#4}}}}
\newcommand{\InstrAB}[2]{\ensuremath{\mathsf{Instr(\mathrm{#1}\!\to\!\mathrm{#2})}}}
\newcommand{\InstrABR}[2]{\ensuremath{\mathsf{Instr_{\mathbb{R}}(\mathrm{#1}\!\to\!\mathrm{#2})}}}
\newcommand{\Instr}[2]{\ensuremath{\mathsf{#1_{\mathsf{#2}}}}}
\newcommand{\InstrA}[1]{\ensuremath{\mathsf{Instr(\mathrm{#1})}}}
\newcommand{\Event}[2]{\ensuremath{\mathsf{Event(\mathrm{#1}\!\to\!\mathrm{#2})}}}
\newcommand{\EventA}[1]{\ensuremath{\mathsf{Event(\mathrm{#1})}}}
\newcommand{\Out}[1]{\ensuremath{\mathsf{#1}}}
\newcommand{\Refi}[1]{\ensuremath{\mathsf{Ref}(\mathscr{#1})}}
\newcommand{\ConvRef}[1]{\ensuremath{\mathsf{ConvRef(\mathscr{#1})}}}

\usepackage{tikz}
\input{tikzit.sty}
\input{style.tikzstyles}

\usepackage{stmaryrd}
\usepackage{xpatch}

\makeatletter
\patchcmd{\@ssect@ltx}
{\addcontentsline{toc}{#1}{\protect\numberline{}#8}}
{}
{}
{}
\makeatother

\makeatletter
\def\@bibdataout@aps{%
	\immediate\write\@bibdataout{%
		@CONTROL{%
			apsrev41Control%
			\longbibliography@sw{%
				,author="08",editor="1",pages="1",title="0",year="1"%
			}{%
				,author="08",editor="1",pages="1",title="",year="1"%
			}%
		}%
	}%
	\if@filesw \immediate \write \@auxout {\string \citation {apsrev41Control}}\fi 
}
\makeatother
